Assessment of certain higher-order structural models based on global approach for bending analysis of curvilinear composite laminates

In this paper, the performance of different structural models based on global approach in evaluating the static response of curvilinear fibre composite laminates is analyzed. A Co shear flexible Quad-8 element developed based on higher-order structural theory is employed for the present study. The structural theory accounting for the realistic variation of displacements through the thickness and the possible discontinuity in the slope at the interface is considered. Four alternate discrete structural models, deduced from the generic structural model by retaining various terms in the displacement functions are examined for their applicability. The accuracy of the present formulation is demonstrated considering the problems for which analytical solutions are available. A systematic numerical study, assuming different ply-angle and lay-up, is conducted in bringing out the influence of various structural models on the static response of composite laminates with curvilinear fibres.

==> staticAna.tex <==
%\subsubsection{Mechanical loading} 
The static analysis is conducted for carbon nanotube reinforced functionally graded sandwich plate with homogeneous core. The following two types of mechanical loading are considered:

\begin{itemize}
\item Mechanical loading
\begin{itemize}
\item Sinusoidal loading: $q(x,y) = q_o \sin \frac{\pi x}{a} \sin \frac{\pi y}{b}$,
\item Uniformly distributed loading: $q(x,y) = q_o$.
\end{itemize}
\item Thermal loading: $T(x,y) = T_o \left( \frac{2z}{h} \right) \sin \frac{\pi x}{a} \sin \frac{\pi y}{b}$
\end{itemize}
where $q_o$ and $T_o$ are the amplitude of the mechanical load and the thermal load, respectively. The physical quantities are nondimensionalized by relations, unless stated otherwise:
\begin{align}
\renewcommand{\arraystretch}{2}
(\overline{u},\overline{v}) &= \frac{100E_{_H}}{q_o h S^3}(u,v) \nonumber \\
\overline{w} &= \frac{100E_H}{q_o h S^4}w \nonumber \\
\overline{\sigma}_{xx} &= \frac{\sigma_{xx}}{q_oS^2} \nonumber \\
\overline{\sigma}_{xz} &= \frac{\sigma_{xz}}{q_oS}
\end{align}
for the applied mechanical load and by
\begin{align}
\renewcommand{\arraystretch}{2}
(\overline{u},\overline{v}) &= \frac{1}{10 h \alpha_H T_o S}(u,v) \nonumber \\
\overline{w} &= \frac{1}{h \alpha_H T_o h S^4}w\nonumber \\
\overline{\sigma}_{xx} &= \frac{\sigma_{xx}}{100 E_H \alpha_H T_o} \nonumber \\
\overline{\sigma}_{xz} &= \frac{\sigma_{xz}}{10 E_H \alpha_H T_o}
\end{align}
for the applied thermal load, where the $E_{_H}, \alpha_{_H}$ are the Young's modulus and the co-efficient of thermal expansion corresponding to the homogeneous core, evaluated at $T_o=$ 300K and $S=a/h$.


Before proceeding to the detailed analysis of the static response of the sandwich plate for the applied mechanical load, the present formulation is validated against available solutions in the literature.  In this case, only one layer is considered. The CNTs are either uniformly distributed or functionally graded along the thickness direction, given by: 
\begin{equation}
V_{\rm CN}(z)  = \left\{ \begin{array}{cl} V_{\rm CN}^\ast &\textup{UD} \\ \left(1 + \frac{2z}{h} \right) V_{\rm CN}^\ast & \textup{FG-V Type} \\ 2\left(\frac{2|z|}{h} \right) V_{\rm CN}^\ast & \textup{FG-X Type} \end{array} \right.
\end{equation}
The effective material properties, viz., Young's modulus, Poisson's ratio and the mass density are estimated from \Eref{eqn:effecprop}. The effect of type of CNT volume fraction distribution is also considered. PmPV~\cite{zhulei2012} is considered as the matrix with material properties: $E_m=$ 2.1 GPa at room temperature (300K), $\nu_m=$ 0.34. The SWCNTs are chosen as the reinforcements and the material properties for the SWCNT are taken from~\cite{zhulei2012} and given in Table \ref{table:cntproperty}. The CNT efficiency parameters $\eta_j$ are determined according to the effective properties of CNTRCs available by matrching the Young's moduli $E_1$ and $E_2$ with the counterparts computed by rule of mixtures. In this study, the efficiency parameters are: $\eta_1=$ 0.149 and $\eta_2=$ 0.934 for the case of $V_{\rm CN}^\ast=$ 0.11; $\eta_1=$ 0.150 and $\eta_2=$ 0.941 for the case of $V_{\rm CN}^\ast=$ 0.14 and $\eta_1=$ 0.149 and $\eta_2=$ 1.381 for the case of $V_{\rm CN}^\ast=$ 0.17. It is assumed that $\eta_2=\eta_3$ for this study.
